Confidence-Based Mesh Extraction from 3D Gaussians

Recently, 3D Gaussian Splatting (3DGS) greatly accelerated mesh extraction from posed images due to its explicit representation and fast software rasterization. While the addition of geometric losses and other priors has improved the accuracy of extracted surfaces, mesh extraction remains difficult in scenes with abundant view-dependent effects. To resolve the resulting ambiguities, prior works rely on multi-view techniques, iterative mesh extraction, or large pre-trained models, sacrificing the inherent efficiency of 3DGS. In this work, we present a simple and efficient alternative by introducing a self-supervised confidence framework to 3DGS: within this framework, learnable confidence values dynamically balance photometric and geometric supervision. Extending our confidence-driven formulation, we introduce losses which penalize per-primitive color and normal variance and demonstrate their benefits to surface extraction. Finally, we complement the above with an improved appearance model, by decoupling the individual terms of the D-SSIM loss. Our final approach delivers state-of-the-art results for unbounded meshes while remaining highly efficient.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


==> sec/3_1_normal.tex <==
\para{Improved Normal Computation}
\begin{wrapfigure}{r}{0.42\textwidth}    \centering
    \includegraphics[width=0.95\linewidth]{figures/normal_figure.pdf}
    \caption{
\textbf{Corrected Normals}:
In contrast to $\msub{\bm{n}}{GOF}$, our normals are consistent with the maximum contribution surface $f(\bf{x}^*)$.
% Left: The normal definition from GOF~\cite{yu2024gof} is inconsistent with the Gaussian geometry, yielding misalignment with the max contribution surface.
% Our normals are consistent with the geometry of the surface, leading to exact alignment between rendered normals and the normal map derived from the depth.
%\todo{Re-Do: smaller, and normals are flipped (actually they're not, but its unclear that ours is on top)}
}
    \label{fig:fixed_normals}
\end{wrapfigure}
Prior work relies on per-primitive normals for geometric regularization.
% However, we find that the definition of the normal of a 3D Gaussian as used by~\cite{Radl2025SOF, yu2024gof} does not align with its geometry.
However, we find that the definition of the normal of a 3D Gaussian as used by~\cite{Radl2025SOF, yu2024gof} is geometrically inconsistent with the rendering process.
The normal definition, as introduced by GOF~\cite{yu2024gof}, is:
%
\begin{equation}
    \msub{\bm{n}}{GOF} = -\bm{\Sigma}^{-1} \bm{d}.
\end{equation}
%
As can be seen in \cref{fig:fixed_normals}, these normals do not align with the surface defined by the maximum contribution $\bm{x}^*$, where the Gaussian is evaluated.
The true maximum contribution surface is an ellipsoid, also intersects the mean $\bm{\mu}$, but, in contrast to GOF, \emph{is not centered on the camera}, but intersects it.
% In fact, the normals follow an ellipsoid, which intersects the mean of the primitive and is centered on the camera.
% However, the maximum contribution surface is an ellipsoid, which also intersects the mean, but \emph{is not centered on the camera}, but intersects it.
We can derive the implicit definition of this surface by inserting $\bm{d} = \bm{x}^* - \bm{o}$ into Eqn.~\eqref{eq:max_point_eval}:
%
\begin{equation}
  f(\bm{x}^*) =(\bm{x}^* - \bm{o})^T \bm{\Sigma}^{-1} (\bm{x}^* - \bm{\mu}),
\end{equation}
%
where the surface is the zero-level set of this function.
By definition, the normal of this surface is the analytical gradient of $f(\bm{x}^*)$:
%
\begin{equation}
    \msub{\bm{n}}{Ours} = \nabla f(\bm{x}^*) = \bm{\Sigma}^{-1} \left(2\bm{x}^* - \bm{\mu}-\bm{o}\right).
\end{equation}
%
In practice, when geometric regularization is used, Gaussians are encouraged to degenerate to disks;
in this case, both normal definitions approach the same results (see the supplementary material for a discussion).
However, we will use $\msub{\bm{n}}{Ours}$ moving forward due to its more grounded geometrical interpretation.
% \todo{Discuss (and optionally prove that the definitions are equivalent for degenerate Gaussians}
% We note that the normal computation, as presented in \gof \cite{yu2024gof} is misaligned with their Ray-Gaussian intersection surface;
% namely, it uses the normal of the intersection plane of the ray $\bm{d}$ in parameter space, which is subsequently transformed back to world space:
% %
% \begin{equation}
%     \msub{\bm{n}}{GOF} = -\bm{\Sigma}^{-1} \bm{d}.
% \end{equation}
% %
% However, this does not respect the geometry of the Gaussians. 
% For a faithful normal, we first define the surface of a 3D Gaussian as the zero-level set of
% %
% \begin{equation}
%     f(\bm{x}) = \bm{x}^T\bm{\Sigma}^{-1}\bm{x} - \bm{x}\bm{\Sigma}^{-1}\bm{\mu}.
% \end{equation}
% %
% We obtain the normal by taking the derivative of $f(\bm{x})$, which results in
% %
% \begin{equation}
%     \msub{\bm{n}}{ours} = \bm{\Sigma}^{-1} \left( 2\bm{x} - \bm{\mu}\right).
% \end{equation}
% %
% See how ours are correct in Fig. {fig:fixed_normals}.
% \todo{Does this even help with optimization? If not for Geometry Reconstruction, then at least for NVS maybe? Also, we have to somewhat note that without this change, the consistency loss is lower-bounded.}

%


==> tables/archive.tex <==
\begin{table}[]
    \centering
    \small
    \setlength{\tabcolsep}{2pt}
\begin{tabular}{lrrrrrrr}
\toprule
 & Barn & Caterpillar & CH & Ignatius & MR & Truck & Average \\
\midrule
w\_conf\_SOF & 0.496 & \cellcolor{tab_color!32}0.448 & \cellcolor{tab_color!15}0.183 & \cellcolor{tab_color!49}0.769 & \cellcolor{tab_color!15}0.320 & \cellcolor{tab_color!49}0.597 & \cellcolor{tab_color!32}0.469 \\
wo\_conf\_SOF & \cellcolor{tab_color!15}0.501 & \cellcolor{tab_color!15}0.436 & 0.122 & \cellcolor{tab_color!15}0.755 & 0.315 & 0.577 & 0.451 \\
DecoupledConvEmbedding & \cellcolor{tab_color!32}0.503 & 0.435 & 0.134 & \cellcolor{tab_color!32}0.761 & \cellcolor{tab_color!15}0.320 & \cellcolor{tab_color!15}0.579 & 0.455 \\
DecoupledConvEmbedding2 & 0.182 & 0.298 & 0.078 & 0.436 & 0.157 & 0.334 & 0.248 \\
DecoupledConvEmbedding3 & \cellcolor{tab_color!49}0.508 & 0.427 & \cellcolor{tab_color!32}0.234 & 0.719 & \cellcolor{tab_color!32}0.323 & 0.574 & \cellcolor{tab_color!15}0.464 \\
DecoupledConvEmbedding4 & 0.221 & 0.345 & 0.015 & 0.510 & 0.209 & 0.381 & 0.280 \\
conf\_lower\_app\_lr & 0.499 & \cellcolor{tab_color!49}0.454 & \cellcolor{tab_color!49}0.294 & 0.703 & \cellcolor{tab_color!49}0.338 & \cellcolor{tab_color!32}0.587 & \cellcolor{tab_color!49}0.479 \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:placeholder}
\end{table}

\begin{table}[]
    \centering
    \small
    \setlength{\tabcolsep}{2pt}
\begin{tabular}{lrrrrrrr}
\toprule
 & BA & CP & CH & IG & MR & TR & Average \\
\midrule
SOF & \cellcolor{tab_color!32}0.538 & 0.410 & 0.292 & \cellcolor{tab_color!15}0.737 & 0.310 & 0.563 & 0.475 \\
VastGaussian (Ours) & \cellcolor{tab_color!49}0.539 & 0.416 & \cellcolor{tab_color!32}0.297 & \cellcolor{tab_color!32}0.740 & 0.320 & 0.570 & \cellcolor{tab_color!49}0.480 \\
VastGaussian (Ours, ignore luminance) & \cellcolor{tab_color!15}0.503 & \cellcolor{tab_color!15}0.430 & \cellcolor{tab_color!49}0.299 & 0.710 & \cellcolor{tab_color!32}0.332 & \cellcolor{tab_color!49}0.590 & \cellcolor{tab_color!15}0.477 \\
Decoupled (ignore luminance term) & 0.499 & \cellcolor{tab_color!32}0.440 & 0.211 & \cellcolor{tab_color!49}0.751 & \cellcolor{tab_color!15}0.327 & \cellcolor{tab_color!15}0.580 & 0.468 \\
Decoupled (lower LR + CONF) & 0.499 & \cellcolor{tab_color!49}0.454 & \cellcolor{tab_color!15}0.294 & 0.703 & \cellcolor{tab_color!49}0.338 & \cellcolor{tab_color!32}0.587 & \cellcolor{tab_color!32}0.479 \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:placeholder}
\end{table}

\begin{table}[]
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lrrrrrrr}
\toprule
 & Barn & Caterpillar & Courthouse & Ignatius & Meetingroom & Truck & Average \\
\midrule
w\_conf\_SOF & 0.496 & \cellcolor{tab_color!49}0.448 & \cellcolor{tab_color!15}0.183 & \cellcolor{tab_color!32}0.769 & \cellcolor{tab_color!49}0.320 & \cellcolor{tab_color!32}0.597 & \cellcolor{tab_color!15}0.469 \\
wo\_conf\_SOF & \cellcolor{tab_color!15}0.501 & \cellcolor{tab_color!32}0.436 & 0.122 & \cellcolor{tab_color!15}0.755 & \cellcolor{tab_color!32}0.315 & \cellcolor{tab_color!15}0.577 & 0.451 \\
MiLo & \cellcolor{tab_color!49}0.590 & 0.390 & \cellcolor{tab_color!32}0.290 & \cellcolor{tab_color!49}0.780 & 0.260 & \cellcolor{tab_color!49}0.620 & \cellcolor{tab_color!49}0.488 \\
SOF & \cellcolor{tab_color!32}0.535 & \cellcolor{tab_color!15}0.408 & \cellcolor{tab_color!49}0.297 & 0.736 & \cellcolor{tab_color!15}0.309 & 0.558 & \cellcolor{tab_color!32}0.474 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
    \centering
\footnotesize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{lrrrrrrr}
\toprule
 & BA & CP & CH & IG & MR & TR & Avg \\
\midrule
VastGaussian & \cellcolor{tab_color!32}0.538 & 0.410 & 0.292 & 0.737 & 0.310 & 0.563 & 0.475 \\
VastGaussian\_Ours & \cellcolor{tab_color!49}0.539 & 0.416 & 0.297 & 0.740 & 0.320 & \cellcolor{tab_color!49}0.570 & 0.480 \\
D-ConvEmbedding & 0.532 & \cellcolor{tab_color!49}0.429 & 0.245 & \cellcolor{tab_color!32}0.751 & 0.315 & 0.556 & 0.471 \\
D-VastGaussianNet\_Lum & 0.533 & 0.421 & 0.297 & \cellcolor{tab_color!15}0.747 & 0.331 & \cellcolor{tab_color!32}0.569 & \cellcolor{tab_color!15}0.483 \\
D-VastGaussianNet\_Full & 0.534 & \cellcolor{tab_color!49}0.429 & \cellcolor{tab_color!15}0.298 & 0.742 & \cellcolor{tab_color!49}0.338 & \cellcolor{tab_color!15}0.568 & \cellcolor{tab_color!32}0.485 \\
D-VastGaussianNet\_Lum\_Detach & \cellcolor{tab_color!15}0.535 & \cellcolor{tab_color!15}0.426 & \cellcolor{tab_color!49}0.313 & \cellcolor{tab_color!49}0.757 & \cellcolor{tab_color!15}0.332 & 0.567 & \cellcolor{tab_color!49}0.488 \\
D-VastGaussianNet\_NoLum & 0.532 & 0.422 & \cellcolor{tab_color!32}0.302 & 0.736 & \cellcolor{tab_color!32}0.334 & 0.559 & 0.481 \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:placeholder}
\end{table}

\begin{tabular}{lrrrr}
\toprule
 & Caterpillar & Meetingroom & Truck & Average \\
\midrule
1\_dec\_app & 0.392 & 0.283 & \cellcolor{tab_color!15}0.533 & \cellcolor{tab_color!15}0.403 \\
2\_conv\_app & \cellcolor{tab_color!15}0.415 & 0.245 & 0.529 & 0.396 \\
3\_no\_app & 0.389 & \cellcolor{tab_color!15}0.284 & \cellcolor{tab_color!15}0.533 & 0.402 \\
4\_conv\_app\_w\_latent & \cellcolor{tab_color!32}0.416 & \cellcolor{tab_color!32}0.306 & \cellcolor{tab_color!32}0.541 & \cellcolor{tab_color!32}0.421 \\
5\_conv\_w\_ssim & \cellcolor{tab_color!49}0.432 & \cellcolor{tab_color!49}0.312 & \cellcolor{tab_color!49}0.564 & \cellcolor{tab_color!49}0.436 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrr}
\toprule
 & scan24 & scan37 & scan63 & Average \\
\midrule
1\_dec\_app & \cellcolor{tab_color!15}0.554 & 0.808 & 1.381 & 0.914 \\
3\_no\_app & \cellcolor{tab_color!32}0.549 & \cellcolor{tab_color!15}0.767 & \cellcolor{tab_color!15}1.281 & \cellcolor{tab_color!15}0.866 \\
4\_conv\_app\_w\_latent & \cellcolor{tab_color!49}0.530 & \cellcolor{tab_color!32}0.705 & \cellcolor{tab_color!32}1.113 & \cellcolor{tab_color!32}0.783 \\
5\_conv\_w\_ssim & 0.556 & \cellcolor{tab_color!49}0.662 & \cellcolor{tab_color!49}1.013 & \cellcolor{tab_color!49}0.743 \\
\bottomrule
\end{tabular}
